Surrogate Model-Based Explainability Methods for Point Cloud NNs

In the field of autonomous driving and robotics, point clouds are showing their excellent real-time performance as raw data from most of the mainstream 3D sensors. Therefore, point cloud neural networks have become a popular research direction in recent years. So far, however, there has been little discussion about the explainability of deep neural networks for point clouds. In this paper, we propose a point cloud-applicable explainability approach based on local surrogate model-based method to show which components contribute to the classification. Moreover, we propose quantitative fidelity validations for generated explanations that enhance the persuasive power of explainability and compare the plausibility of different existing point cloud-applicable explainability methods. Our new explainability approach provides a fairly accurate, more semantically coherent and widely applicable explanation for point cloud classification tasks. Our code is available at https://github.com/Explain3D/LIME-3D

==> notes/16_Aug_Note.tex <==
Gerneral:
- We could already update our Axiv Version with this one, right?
Sure!


Abstract:
☑️* we propose a point cloud ... -> we propose a point cloud-applicable expl. approach or ... propose point ... approaches - plural or singular?

Introduction:
☑️* Despite ... the industry -> in industry
☑️* security-critical -> safety-critical?
☑️* remain black boxes -> .. black-boxes
☑️* Therefore, it indicates... -> This calls for the development, of ... or This indicates an ...
☑️* With the help of ... -> With the help of explanationS
* ... cases trough .. -> ... cases through our proposed methods/approaches or through the proposed approach? singular vs plural

Related Work:
☑️* Why do we have subsubsections like 2.0.1 instead of 2.1, I think this is not allowed? If this is to save space I would instead again use the titles directly in the text mark them in bold ot italic as in paper 2. This will be fine since it's the related work section!
2.0.1
    ☑️* two times italic "local surrogate model-based" last paragraph.
    ☑️* I would add one short sentence at the end of 2.0.1 that this work focuses on sur.model-based methods and why. If we have space
2.0.2
    ☑️* Point clouds  have ... due to its --> .. due to their
    ☑️* Add one half sentence at the end, that this Modenet40 Benchmark will be also used in our Experiment section.
2.0.3
    ☑️* PointHop Unit -> PointHop UnitS
2.0.4
    ☑️* Title: varification -> verification
    ☑️* the varified prediction -> the verified ...
    
Explainability Approaches for Point Clouds
3.1.1
    * Algorithm 1: 
        ☑️* I would put the comments e.g.: "Indicates each point..." above the related lines instead of behind them, this makes it more readable. 
        ☑️* Maybe you could also find a shorter name for line 7 e.g. "EDMatrix <- euclidDist(P, Cen)", so it might fit in one line, but its also ok like this.
    ☑️*such that for each ... -> such that what? Maybe missing verb before p € Ci? 
3.2.2
    ☑️* Additional measuring methodo... -> Add.. m.. m.. are required for ..

Experiments
☑️Fig 1: if more space is needed you could minimize the airplane pics to fit to one line, and maybe you need this space?
4.1.1
    ☑️(Added in the start of 4.2, maybe this looks more nature..)* Maybe reference to Table S1 in supplementary at the end regarding a proof for the processing time issue but this is optional
4.2.1
    ☑️* The local fidelity metrics -> Local fidelity metrics : plural, right?
    ☑️* black box -> black-box
    ☑️* table 1 compares ... -> Table 1 compares the local fidelity (see Sec 3.2.1) of different tricks????. First you should somehow link what D and R means which is explained in Sec 3.2.1. Second, what do you mean with "tricks" "mechanics" (also used in caption of Tbl 3)? Is this the usual term? Maybe mechanisms, methods?? Third, are the short version names like "VISF" somewhere defined in Section 3, maybe use same names in Sec 3 or reference/mark them, I see FPS is defined in Algo 1, but this was for preprocessing?
    ☑️* According to ... -> According to ... our .. (FPS + VISF) - we should reference which column/raw you mean, I guess the last one. 
4.2.2
    ☑️* dominates the rests -> delete "the rests" : The proposed method (FPS.+VISF.) dominates which is ...
    ☑️* Reference to Figure 2 maybe earlier when you mention tbl2. 
    ☑️* Figure 2:
        * please mention what the "average score" y-axis is and reference where it is defined! Is there a reason why you deleted the variance? In the supplementary Figure S1 you mention that the lines are the means and variances in the caption, but the variances are not shown. I would show the variances in both pics. But you are the expert, maybe you have a reason. But in general showing the variance is more fair.
        * You could add "positive contribution points" in the legend instead of only "positive" if you want to shorten the caption or save space. same for negative and random
    ☑️*Tbl 3: caption : the plau... -> Plausibility p of different methods for explanation quality enhancement. 

Supplementary:
☑️* Fig S2 caption: -> white-space missing: p15, p3 
* Fig S1 caption: -> variances are not shown! You might want to add them



